Dual Caption Preference Optimization for Diffusion Models

Recent advancements in human preference optimization, originally developed for Large Language Models (LLMs), have shown significant potential in improving text-to-image diffusion models. These methods aim to learn the distribution of preferred samples while distinguishing them from less preferred ones. However, within the existing preference datasets, the original caption often does not clearly favor the preferred image over the alternative, which weakens the supervision signal available during training. To address this issue, we introduce Dual Caption Preference Optimization (DCPO), a data augmentation and optimization framework that reinforces the learning signal by assigning two distinct captions to each preference pair. This encourages the model to better differentiate between preferred and less-preferred outcomes during training. We also construct Pick-Double Caption, a modified version of Pick-a-Pic v2 with separate captions for each image, and propose three different strategies for generating distinct captions: captioning, perturbation, and hybrid methods. Our experiments show that DCPO significantly improves image quality and relevance to prompts, outperforming Stable Diffusion (SD) 2.1, SFT_Chosen, Diffusion-DPO, and MaPO across multiple metrics, including Pickscore, HPSv2.1, GenEval, CLIPscore, and ImageReward, fine-tuned on SD 2.1 as the backbone.

==> Tables/support_hyphotesis1.tex <==
\begin{wraptable}{r}{0.5\linewidth}
\small
\centering

\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lcccc@{}}
\toprule
\multicolumn{1}{c}{\textbf{}} & \textbf{\stackanchor{\textbf{Captioning}}{\textbf{LLaVA}}} & \textbf{\stackanchor{\textbf{Perturbed}}{\textbf{Weak}}} & \textbf{\stackanchor{\textbf{Perturbed}}{\textbf{Medium}}} & \textbf{\stackanchor{\textbf{Perturbed}}{\textbf{Strong}}} \\ 
\midrule
\(\Delta \mu(z^w,z^l)\) & 4.37 & 6.44 & 6.76 & 8.29 \\
Pickscore & 20.46 & 20.58 & 20.57 & 20.58 \\
HPSv2.1 & 25.10 & 25.70 & 25.62 & 25.43 \\
ImageReward & 56.5 & 58.1 & 58.2 & 57.9 \\
CLIPscore & 27.00 & 27.15 & 27.13 & 27.21 \\
GenEval & 49.71 & 50.60 & 51.00 & 49.93 \\
\midrule
Average & 25.75 & 36.43 & \textbf{36.50} & 36.21 \\

\bottomrule
\end{tabular}%
\caption{hyphotesis 1 ..}
\label{tab:hyphotesis1}
}
\end{wraptable}






